Atalaya at TASS 2019: Data Augmentation and Robust Embeddings for Sentiment Analysis

In this article we describe our participation in TASS 2019, a shared task aimed at the detection of sentiment polarity of Spanish tweets. We combined different representations such as bag-of-words, bag-of-characters, and tweet embeddings. In particular, we trained robust subword-aware word embeddings and computed tweet representations using a weighted-averaging strategy. We also used two data augmentation techniques to deal with data scarcity: two-way translation augmentation, and instance crossover augmentation, a novel technique that generates new instances by combining halves of tweets. In experiments, we trained linear classifiers and ensemble models, obtaining highly competitive results despite the simplicity of our approaches.

==> source/other_ideas.tex <==
\subsection{Other Ideas}
\label{sec:other}

We tried several other ideas with different levels of success.
In this section we briefly describe some of them.

**Bagging**

Data Augmentation using Embedding Similarities

testing time augmentation (TTA)

Contextual word embeddings:
We trained an ULMFiT language model using our tweet database, and fine-tuned it for sentiment classification using TASS corpora.

Preliminar results using ULMFiT standalone, and using ULMFiT vectors as features for our main system.

We trained a Multi-Layer Perceptron

neural MLP (pytorch).

